AdaCLIP: Adapting CLIP with Hybrid Learnable Prompts for Zero-Shot Anomaly Detection

Zero-shot anomaly detection (ZSAD) targets the identification of anomalies within images from arbitrary novel categories. This study introduces AdaCLIP for the ZSAD task, leveraging a pre-trained vision-language model (VLM), CLIP. AdaCLIP incorporates learnable prompts into CLIP and optimizes them through training on auxiliary annotated anomaly detection data. Two types of learnable prompts are proposed: static and dynamic. Static prompts are shared across all images, serving to preliminarily adapt CLIP for ZSAD. In contrast, dynamic prompts are generated for each test image, providing CLIP with dynamic adaptation capabilities. The combination of static and dynamic prompts is referred to as hybrid prompts, and yields enhanced ZSAD performance. Extensive experiments conducted across 14 real-world anomaly detection datasets from industrial and medical domains indicate that AdaCLIP outperforms other ZSAD methods and can generalize better to different categories and even domains. Finally, our analysis highlights the importance of diverse auxiliary data and optimized prompts for enhanced generalization capacity. Code is available at https://github.com/caoyunkang/AdaCLIP.

==> sources/3-method-backup.tex <==
\section{Method}\label{sec:method}

\subsection{Problem Definition}

Zero-shot anomaly detection is designed to create a versatile model capable of detecting anomalies across a wide range of categories. When presented with an image $\mathbf{I} \in \mathrm{R}^{H \times W \times 3}$ belonging to previously unseen categories, the ZSAD model is expected to generate an anomaly score $S \in [0, 1]$ for the given image, indicating the degree of anomaly exhibited by the given image. In addition to the anomaly score, the model needs to produce an anomaly map $\mathbf{M} \in [0, 1]$, precisely pinpointing the locations of anomalies within the input image. The ZSAD task holds potential due to its adaptability across diverse domains. However, it is challenging as there is a lack of prior information regarding the target categories. 

\subsection{Revisiting CLIP for Anomaly Detection}
Existing ZSAD methods~\cite{WinClip,VAND} predominantly rely on a robust VLM, CLIP~\cite{clip}, for their anomaly detection capacity on novel categories. CLIP consists of an image encoder $\mathcal{V}$ and a text encoder $\mathcal{L}$, typically employing a ViT~\cite{liu2021swin} architecture. CLIP can extract vision and text features in a unified representation space. 

\subsubsection{Extracting Image Representation} 

Image encoder $\mathcal{V}$ consists of $K$ transformer layers $\{ \mathcal{V}_{i=1}^K\}$. For a given image $\mathbf{I}$, the image encoder firstly extracts its corresponding patch embeddings $\mathbf{E}_0 \in \mathrm{R}^{M \times d_v}$. Then the $(i+1)^{th}$ transformer layer $\mathcal{V}_{i+1}$ processes patch embeddings $\mathbf{E}_i$ along with a learnable class token $c_i$ and sequentially processed through $K$ transformer layers,


\begin{equation}
[c_i, \mathbf{E}_i] = \mathcal{V}_i([c_{i-1}, \mathbf{E}_{i-1}]) \quad i = 1,2,\ldots,K.
\end{equation}

To obtain the final image representation $\mathbf{F}^I$, the class token $c_K$ of the last transformer layer $\mathcal{V}_K$ is projected to a common V-L latent representation space via $\text{ImageProj}(\cdot)$,

\begin{equation}
\mathbf{F}^I = \text{ImageProj}(c_K) \quad \mathbf{F}^I \in \mathbb{R}^{d_u}
\end{equation}
where ${d_u}$ is the dimension of the common representation space.

\subsubsection{Extracting Text Representation}

CLIP text encoder generates feature representations for text description like ``\texttt{A photo of a [cls]}'' by tokenizing the words and projecting them to word embeddings $W_0 \in \mathrm{R}^{N\times d_l}$. At each stage, $W_i$ is input to the $(i + 1)^th$ textual transformer layer $\mathcal{L}_{i+1}$,

\begin{equation}
[W_i] = \mathcal{L}_i(W_{i-1}) \quad i = 1,2,\ldots,K.
\end{equation}

The final text representation $f^L$ is obtained by projecting the text embeddings corresponding to the last token of the last transformer block $\mathcal{L}_{K}$ to a common V-L latent embedding space via $\text{TextProj}(\cdot)$,

\begin{equation}
f^L = \text{TextProj}(W_K) \quad f^L \in \mathbb{R}^{d_u}
\end{equation}


\subsubsection{Anomaly Detection}

Existing CLIP-based ZSAD methods~\cite{WinClip,VAND} utilize the similarities between vision and normal/abnormal representations to yield anomaly scores. Formally, normal and abnormal text templates are defined with normal and abnormal descriptions, respectively, such as ``\texttt{A photo of a normal [cls]}'' and ``\texttt{A photo of a damaged [cls]}''. Then CLIP is employed to extract the textual representation $\mathbf{F}^L\in \mathbb{R}^{2 \times d_u}$ for the normal/abnormal text templates, with $\mathbf{F}^L_{0,:}$ and $\mathbf{F}^L_{1,:}$ for normal and abnormal descriptions, respectively. CLIP also extracts image representations $\mathbf{F}^I$. Then the anomaly score is derived from the similarity between these representations,

\begin{equation}
\label{eq:AS}
S = \text{Softmax}(\langle \mathbf{F}^I, {F^L} \rangle)
\end{equation}

Here, $\langle \cdot,\cdot \rangle$ denotes the cosine similarity calculation function, and $S_{(1)}$ signifies the likelihood of the testing image being abnormal.

Anomaly localization further exploits the similarity between patch embeddings and language representations to derive pixel-wise anomaly maps. Specifically, the image embeddings undergo projection to the common vision-language representation space through a projection layer $\text{P}(\cdot)$:

\begin{equation}
\mathbf{M}_i = \text{Reshape}(\text{Softmax}(\langle \text{P}(\mathbf{E}_i), {F^L} \rangle))
\end{equation}

In this context, the $\text{Reshape}(\cdot)$ function translates the similarity sequence into the original shape of the input image, and $\mathbf{M}_{(x,y,1)}$ indicates the likelihood of the entity $(x,y)$ in the testing image being abnormal. A multi-hierarchy strategy is usually employed to boost the pixel-level anomaly detection performance, 

\begin{equation}
\label{eq:AM}
\mathbf{M} = \sum_{i \in \mathcal{H}} \mathbf{M}_i
\end{equation}
Here, $\mathcal{H}$ denotes the indexes of selected layers.

\subsubsection{Analysis}
Existing CLIP-based ZSAD methods have demonstrated some effectiveness in detecting anomalies in novel categories. However, as illustrated in Fig.\ref{fig:teaser}, their distinguishment deteriorates when faced with categories that exhibit large variances. This decline can be attributed to their reliance on fixed representation spaces. While fixed representation spaces may perform well on encountered data types or patterns, they may struggle when confronted with new, unseen anomalous patterns. Such spaces might overly depend on specific features in the training data, resulting in reduced generalization ability when confronted with new or different types of data.

\begin{figure*}
    \centering
    \includegraphics[width=1.\linewidth]{figures/figure3.png}
    \caption{framework of the proposed method.}
    \label{fig:framework}
\end{figure*}

\subsection{Overview of AdaCLIP}

This study endeavors to formulate a representation space adaptable at test time for zero-shot anomaly detection, thereby enhancing its efficacy in handling novel categories. The proposed approach, AdaCLIP, achieves this by generating instance-conditioned prompts through an Instance-Conditioned Prompt Generator during test time to govern the encoders, as illustrated in Fig.~\ref{fig:framework}. While these generated prompts enhance the ability of the model to capture abnormality variances, they may be susceptible to fragility due to inherent noise in the generation process. To mitigate this, task-conditioned prompts are introduced to provide a robust estimation foundation, thereby reducing the impact of noise. With the incorporation of both instance-conditioned and task-conditioned prompts, AdaCLIP enables the CLIP representation space to concurrently encompass both the variance and invariance associated with abnormalities. AdaCLIP introduces prompts on both the image and text encoders to comprehensively prompt the encoders. Regarding calculating the anomaly score $S$, AdaCLIP employs a Hybrid Semantic Fusion model, fusing semantics from multiple layers to capture fine-grained and global information, consequently yielding enhanced anomaly detection performance.

\subsection{Hybrid Multi-modality Prompting}
The hybrid multi-modality prompting method encompasses multi-modality instance- and task-condition prompts, constituting a comprehensive approach to prompt the CLIP model. This method is designed to generate an optimized representation space specifically tailored for the anomaly detection task on the target category, thus simultaneously capturing both invariances and variances of abnormalities.


\subsubsection{Multi-modality Prompting}

Existing ZSAD methods, such as VAND~\cite{VAND}, have leveraged projection layers to adapt the CLIP representation space using auxiliary data. While projection layers behind the output of CLIP can adjust the representation space, prompting learning has been demonstrated to be more effective~\cite{CoOp,coCoOp} in adapting such spaces. Prompting learning typically involves adding learnable tokens to the input or inside the model, which are optimized during training, while the original parameters remain frozen. These added learnable tokens are lightweight compared to the original parameters of CLIP, thus not affecting the generality of CLIP. Taking vision prompting learning~\cite{Zha_2023_ICCV,MaPLe} as an example, $L$ learnable tokens $\mathbf{P} \in \mathrm{R}^{L \times d_v}$ are introduced in the first $D$ layers of the vision branch.

\begin{equation}
[c_i, \mathbf{E}_i, \_] = \mathcal{V}_i([c_{i-1}, \mathbf{E}_{i-1}, \mathbf{P}_{i-1}]) \quad i = 1,2,\ldots,D.
\end{equation}

Here $[\cdot, \cdot]$ refers to the concatenation operation. After $D^{th}$ transformer layer, the subsequent layers process the previous layer prompts,
\begin{equation}
[c_j, \mathbf{E}_j, \mathbf{P}_{j}] = \mathcal{V}_j([c_{j-1}, \mathbf{E}_{j-1}, \mathbf{P}_{j-1}]) \quad j = D+1,\ldots,K.
\end{equation}

Despite the effectiveness of current prompting methods in adjusting CLIP, they primarily concentrate on prompting either the text or the vision encoder exclusively. In contrast, AdaCLIP suggests prompting both branches for a more thorough adaptation. Alongside the vision branch, AdaCLIP introduces $L$ learnable tokens $\widetilde{\mathbf{P}} \in \mathrm{R}^{L \times d_l}$ within the initial $D$ layers of the text branch.

\begin{equation}
[\mathbf{W}_i, \_] = \mathcal{L}_i([\mathbf{W}_{i-1}, \widetilde{\mathbf{P}}_{i-1}]) \quad i = 1,2,\ldots,D.
\end{equation}

\begin{equation}
[\mathbf{W}_j, \widetilde{\mathbf{P}}_{j}] = \mathcal{L}_j([\mathbf{W}_{j-1}, \widetilde{\mathbf{P}}_{j-1}]) \quad j = D+1,\ldots,K.
\end{equation}


\subsubsection{Instance-Conditioned Prompting}

Prompts play a crucial role in regulating the functionality of models~\cite{SAA,coCoOp}, serving as a mechanism to guide their performance. In this context, AdaCLIP introduces an instance-conditioned prompting method aimed at generating prompts based on input samples. This approach dynamically adjusts models to better suit the characteristics of the inputs, thereby enhancing the model's adaptability to new, unseen data, or anomalous patterns. Formally, it can be expressed as follows,

\begin{equation}
\label{eq:generator}
\mathbf{P}_{i}^{IC}, \widetilde{\mathbf{P}}_{i}^{IC} = \text{G}(\mathbf{I})
\end{equation}
where $\text{G}(\cdot)$ denotes a lightweight instance-conditioned prompts generator, and $\mathbf{P}_{i}^{IC} \in \mathrm{R}^{L \times d_v}, \widetilde{\mathbf{P}}_{i}^{IC} \in \mathrm{R}^{L \times d_l}$ are generated instance-conditioned vision and text prompts.

The introduction of dynamic prompts provides the model with heightened flexibility. This adaptability proves essential when confronting novel situations or encountering anomalous patterns. Moreover, the synergy of these dynamic prompts empowers the model to not only learn invariances of abnormalities but also adapt to the specific variances of each individual sample.

The significance of instance-conditioned prompts becomes apparent in their role as facilitators of "customized" adjustments for individual inputs. This tailored approach proves particularly beneficial in handling individual differences and special cases, a critical aspect when dealing with diverse datasets and domains. In essence, the incorporation of instance-conditioned prompts equips the model with the means to navigate the intricacies of diverse data, enhancing its overall efficacy in anomaly detection.

\subsubsection{Task-Conditioned Prompting}
While instance-conditioned prompting contributes to a dynamic representation space, it is not without its challenges, particularly regarding the susceptibility to disturbances inherent in the prompting generation process. Specifically, these prompts rely on complex generation processes through the generator $\text{G}(\cdot)$, which can introduce noise, particularly when the input data itself is noisy or irregular. This noise may result in considerable fluctuations in model predictions between individual samples, undermining consistency. 
In response to these challenges, this study introduces a task-conditioned prompting technique aimed at establishing a foundational optimizing direction. The primary objective is to mitigate the influence of inherent noise in instance-conditioned prompting, thereby enhancing the reliability and robustness of the model's responses. 

In contrast to instance-conditioned prompts generated dynamically, these task-conditioned prompts $\mathbf{P}_{i}^{TC} \in \mathrm{R}^{L \times d_v}, \widetilde{\mathbf{P}}_{i}^{TC} \in \mathrm{R}^{L \times d_l}$ are optimized in the training process and fixed during testing. Task-conditioned prompts serve as the cornerstone for baseline representation space building within the model. These prompts capture universal invariances of abnormalities, facilitating a robust mechanism for generalization to new data and unseen scenarios. The universality they provide is crucial for handling novel categories and ensuring the model's ability to generalize. Hence, AdaCLIP combines instance- and task-conditioned prompts for more reliable and robust ZSAD,

\begin{equation}
\mathbf{P}_{i} = \mathbf{P}_{i}^{IC} + \mathbf{P}_{i}^{TC}, \widetilde{\mathbf{P}}_{i} = \widetilde{\mathbf{P}}_{i}^{IC} + \widetilde{\mathbf{P}}_{i}^{TC}
\end{equation}
where $\mathbf{P}_{i},  \widetilde{\mathbf{P}}_{i}$ are the final utilized prompts for the vision and text encoders, respectively.

% Instance-conditioned prompts empower the model to provide customized representation space for individual inputs, capturing the variances in abnormalities. This capability allows the model to discern unique features in individual samples, particularly those exhibiting uncommon or entirely unseen abnormal patterns in the training data. On the other hand, task-conditioned prompts are responsible for learning invariances of abnormalities that persist throughout the entire training dataset. This global perspective is crucial for establishing a solid foundation and promoting generalization in the model. The combined use of instance- and task-conditioned parameters presents a stable and flexible framework for ZSAD. AdaCLIP harnesses the advantages of both parameter types, enabling the model to effectively handle diverse data types while maintaining high accuracy and robustness.



\subsection{Hybrid Semantic Fusion}

Concerning the computation of anomaly scores $S$, prevailing anomaly detection methods typically either utilize the maximum value within anomaly maps $\mathbf{M}$~\cite{CDO,2023CaiDis} or derive scores based on the global image embedding~\cite{VAND, WinClip}. However, the maximum-value-based approach has shown vulnerability in scenarios with false alarms~\cite{CDO}, while the global embeddings often lack robust fine-grained semantics, leading to potential inaccuracies in anomaly scores~\cite{VAND}. Therefore, AdaCLIP proposes a Hybrid Semantic Fusion (HSF) module to calculate anomaly scores based on both fine-grained local and global semantics, amalgamating the strengths of both strategies. Specifically, as Fig.~\ref{fig:HSF} shows, HSF extracts local semantics through the embeddings that are most likely to be abnormal. Then, HSF fuses these fine-grained semantics with image representations that contain global semantics.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/figure4.png}
    \caption{details of HSF.}
    \label{fig:HSF}
\end{figure}

\subsubsection{Local Semantic Extraction}

Vision embeddings with relatively high anomaly scores are more likely to indicate abnormalities~\cite{CDO, wang2021student}. In simpler terms, these embeddings encapsulate intricate semantics associated with anomalies. To distill these semantics, HSF selects the top-K embeddings based on the corresponding anomaly map in individual layers. These selected embeddings typically represent various candidates for anomaly regions. However, directly fusing these embeddings may diminish the significance of regions with smaller scales. In order to apply similar attention to different regions, HSF proposes to extract their cluster centroids as the final embeddings for local semantics,

\begin{equation}
\label{eq:fusion}
\mathcal{S}_i = \text{Kmeans}(\text{TopK}(\mathbf{E}_i  | \mathbf{M}_{(x,y,1)}))
\end{equation}

Here, $\text{TopK}(\mathbf{E}_i  | \mathbf{M}_{(x,y,1)})$ denotes the selection of the top-K embeddings with the highest abnormal scores conditioned on anomaly maps $\mathbf{M}_{(x,y,1)}$. $\text{Kmeans}(\cdot)$ represents the Kmeans clustering algorithm, and $\mathcal{S}_i$ is the generated index set for individual clusters.

Subsequently, the $j$-th cluster centroid in the $i$-th layer is calculated by averaging its corresponding embeddings,

\begin{equation}
\mathbf{C}_{i,j} = \frac{1}{|\mathcal{S}_{i,j}|} \sum_{k \in \mathcal{S}_{i,j}}{\mathbf{E}_{i,k}}
\end{equation}

The local semantic ${\mathbf{C}}_i$ for the $i$-th layer is obtained by averaging the cluster centroids,

\begin{equation}
{\mathbf{C}}_{i} = \frac{1}{N_c} \sum_{j = 0}^{N_c}{\mathbf{C}_{i,j}}
\end{equation}


\subsubsection{Local-Global Semantic Aggregation}
Image representations $\mathbf{F}^I$ encapsulate global semantics for the inputs, proving beneficial for anomaly score calculation~\cite{WinClip}. In this context, HSF integrates global image representations with the previously discussed local semantics to create enriched image representations. Specifically, the local semantics are projected to the common V-L representation space through the aforementioned projection layer $\text{P}(\cdot)$ before the aggregation, 

\begin{equation}
\widetilde{\mathbf{F}}^I = \mathbf{F}^I + \sum_{i \in \mathcal{H}} {\text{P}({\mathbf{C}}_{i})}
\end{equation}

Here, $\widetilde{\mathbf{F}}^I$ signifies the resulting hybrid semantic representation, subsequently employed for calculating anomaly scores using Equation~\ref{eq:AS}.

\subsection{Training and Inference}

During the training stage, the parameters of the CLIP model are frozen. AdaCLIP only optimizes the hybrid multi-modality prompts and the project layers. Focal loss~\cite{focalloss} is utilized for anomaly score calculation.  Focal loss and dice loss~\cite{diceloss} are employed to produce reliable anomaly maps. During inference, the anomaly score and maps are derived from Equations~\ref{eq:AS} and ~\ref{eq:AM}, respectively.




With patch embeddings, image embedding


Zero-shot anomaly detection is designed to create a versatile model capable of detecting anomalies across a wide range of categories. When presented with an image $\mathbf{I} \in \mathrm{R}^{H \times W \times 3}$ belonging to previously unseen categories, the ZSAD model is expected to generate an anomaly score $S \in [0, 1]$ for the given image, indicating the degree of anomaly exhibited by the given image. In addition to the anomaly score, the model needs to produce an anomaly map $\mathbf{M} \in [0, 1]$, precisely pinpointing the locations of anomalies within the input image. The ZSAD task holds potential due to its adaptability across diverse domains. However, it is challenging as there is a lack of prior information regarding the target categories. 

\subsection{Revisiting CLIP for Anomaly Detection}
Existing ZSAD methods~\cite{WinClip,VAND} predominantly rely on a robust VLM, CLIP~\cite{clip}, for their anomaly detection capacity on novel categories. CLIP consists of an image encoder $\mathcal{V}$ and a text encoder $\mathcal{L}$, typically employing a ViT~\cite{liu2021swin} architecture. CLIP can extract vision and text features in a unified representation space. 

\subsubsection{Extracting Image Representation} 

Image encoder $\mathcal{V}$ consists of $K$ transformer layers $\{ \mathcal{V}_{i=1}^K\}$. For a given image $\mathbf{I}$, the image encoder firstly extracts its corresponding patch embeddings $\mathbf{E}_0 \in \mathrm{R}^{M \times d_v}$. Then the $(i+1)^{th}$ transformer layer $\mathcal{V}_{i+1}$ processes patch embeddings $\mathbf{E}_i$ along with a learnable class token $c_i$ and sequentially processed through $K$ transformer layers,


\begin{equation}
[c_i, \mathbf{E}_i] = \mathcal{V}_i([c_{i-1}, \mathbf{E}_{i-1}]) \quad i = 1,2,\ldots,K.
\end{equation}

To obtain the final image representation $\mathbf{F}^I$, the class token $c_K$ of the last transformer layer $\mathcal{V}_K$ is projected to a common V-L latent representation space via $\text{ImageProj}(\cdot)$,

\begin{equation}
\mathbf{F}^I = \text{ImageProj}(c_K) \quad \mathbf{F}^I \in \mathbb{R}^{d_u}
\end{equation}
where ${d_u}$ is the dimension of the common representation space.

\subsubsection{Extracting Text Representation}

CLIP text encoder generates feature representations for text description like ``\texttt{A photo of a [cls]}'' by tokenizing the words and projecting them to word embeddings $W_0 \in \mathrm{R}^{N\times d_l}$. At each stage, $W_i$ is input to the $(i + 1)^th$ textual transformer layer $\mathcal{L}_{i+1}$,

\begin{equation}
[W_i] = \mathcal{L}_i(W_{i-1}) \quad i = 1,2,\ldots,K.
\end{equation}

The final text representation $f^L$ is obtained by projecting the text embeddings corresponding to the last token of the last transformer block $\mathcal{L}_{K}$ to a common V-L latent embedding space via $\text{TextProj}(\cdot)$,

\begin{equation}
f^L = \text{TextProj}(W_K) \quad f^L \in \mathbb{R}^{d_u}
\end{equation}


\subsubsection{Anomaly Detection}

Existing CLIP-based ZSAD methods~\cite{WinClip,VAND} utilize the similarities between vision and normal/abnormal representations to yield anomaly scores. Formally, normal and abnormal text templates are defined with normal and abnormal descriptions, respectively, such as ``\texttt{A photo of a normal [cls]}'' and ``\texttt{A photo of a damaged [cls]}''. Then CLIP is employed to extract the textual representation $\mathbf{F}^L\in \mathbb{R}^{2 \times d_u}$ for the normal/abnormal text templates, with $\mathbf{F}^L_{0,:}$ and $\mathbf{F}^L_{1,:}$ for normal and abnormal descriptions, respectively. CLIP also extracts image representations $\mathbf{F}^I$. Then the anomaly score is derived from the similarity between these representations,

\begin{equation}
\label{eq:AS}
S = \text{Softmax}(\langle \mathbf{F}^I, {F^L} \rangle)
\end{equation}

Here, $\langle \cdot,\cdot \rangle$ denotes the cosine similarity calculation function, and $S_{(1)}$ signifies the likelihood of the testing image being abnormal.

Anomaly localization further exploits the similarity between patch embeddings and language representations to derive pixel-wise anomaly maps. Specifically, the image embeddings undergo projection to the common vision-language representation space through a projection layer $\text{P}(\cdot)$:

\begin{equation}
\mathbf{M}_i = \text{Reshape}(\text{Softmax}(\langle \text{P}(\mathbf{E}_i), {F^L} \rangle))
\end{equation}

In this context, the $\text{Reshape}(\cdot)$ function translates the similarity sequence into the original shape of the input image, and $\mathbf{M}_{(x,y,1)}$ indicates the likelihood of the entity $(x,y)$ in the testing image being abnormal. A multi-hierarchy strategy is usually employed to boost the pixel-level anomaly detection performance, 

\begin{equation}
\label{eq:AM}
\mathbf{M} = \sum_{i \in \mathcal{H}} \mathbf{M}_i
\end{equation}
Here, $\mathcal{H}$ denotes the indexes of selected layers.

\subsubsection{Analysis}
Existing CLIP-based ZSAD methods have demonstrated some effectiveness in detecting anomalies in novel categories. However, as illustrated in Fig.\ref{fig:teaser}, their distinguishment deteriorates when faced with categories that exhibit large variances. This decline can be attributed to their reliance on fixed representation spaces. While fixed representation spaces may perform well on encountered data types or patterns, they may struggle when confronted with new, unseen anomalous patterns. Such spaces might overly depend on specific features in the training data, resulting in reduced generalization ability when confronted with new or different types of data.

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.\linewidth]{figures/figure3.png}
%     \caption{framework of the proposed method.}
%     \label{fig:framework}
% \end{figure*}

\subsection{Overview of AdaCLIP}

This study endeavors to formulate a representation space adaptable at test time for zero-shot anomaly detection, thereby enhancing its efficacy in handling novel categories. The proposed approach, AdaCLIP, achieves this by generating instance-conditioned prompts through an Instance-Conditioned Prompt Generator during test time to govern the encoders, as illustrated in Fig.~\ref{fig:framework}. While these generated prompts enhance the ability of the model to capture abnormality variances, they may be susceptible to fragility due to inherent noise in the generation process. To mitigate this, task-conditioned prompts are introduced to provide a robust estimation foundation, thereby reducing the impact of noise. With the incorporation of both instance-conditioned and task-conditioned prompts, AdaCLIP enables the CLIP representation space to concurrently encompass both the variance and invariance associated with abnormalities. AdaCLIP introduces prompts on both the image and text encoders to comprehensively prompt the encoders. Regarding calculating the anomaly score $S$, AdaCLIP employs a Hybrid Semantic Fusion model, fusing semantics from multiple layers to capture fine-grained and global information, consequently yielding enhanced anomaly detection performance.

\subsection{Hybrid Multi-modality Prompting}
The hybrid multi-modality prompting method encompasses multi-modality instance- and task-condition prompts, constituting a comprehensive approach to prompt the CLIP model. This method is designed to generate an optimized representation space specifically tailored for the anomaly detection task on the target category, thus simultaneously capturing both invariances and variances of abnormalities.


\subsubsection{Multi-modality Prompting}

Existing ZSAD methods, such as VAND~\cite{VAND}, have leveraged projection layers to adapt the CLIP representation space using auxiliary data. While projection layers behind the output of CLIP can adjust the representation space, prompting learning has been demonstrated to be more effective~\cite{CoOp,coCoOp} in adapting such spaces. Prompting learning typically involves adding learnable tokens to the input or inside the model, which are optimized during training, while the original parameters remain frozen. These added learnable tokens are lightweight compared to the original parameters of CLIP, thus not affecting the generality of CLIP. Taking vision prompting learning~\cite{Zha_2023_ICCV,MaPLe} as an example, $L$ learnable tokens $\mathbf{P} \in \mathrm{R}^{L \times d_v}$ are introduced in the first $D$ layers of the vision branch.

\begin{equation}
[c_i, \mathbf{E}_i, \_] = \mathcal{V}_i([c_{i-1}, \mathbf{E}_{i-1}, \mathbf{P}_{i-1}]) \quad i = 1,2,\ldots,D.
\end{equation}

Here $[\cdot, \cdot]$ refers to the concatenation operation. After $D^{th}$ transformer layer, the subsequent layers process the previous layer prompts,
\begin{equation}
[c_j, \mathbf{E}_j, \mathbf{P}_{j}] = \mathcal{V}_j([c_{j-1}, \mathbf{E}_{j-1}, \mathbf{P}_{j-1}]) \quad j = D+1,\ldots,K.
\end{equation}

Despite the effectiveness of current prompting methods in adjusting CLIP, they primarily concentrate on prompting either the text or the vision encoder exclusively. In contrast, AdaCLIP suggests prompting both branches for a more thorough adaptation. Alongside the vision branch, AdaCLIP introduces $L$ learnable tokens $\widetilde{\mathbf{P}} \in \mathrm{R}^{L \times d_l}$ within the initial $D$ layers of the text branch.

\begin{equation}
[\mathbf{W}_i, \_] = \mathcal{L}_i([\mathbf{W}_{i-1}, \widetilde{\mathbf{P}}_{i-1}]) \quad i = 1,2,\ldots,D.
\end{equation}

\begin{equation}
[\mathbf{W}_j, \widetilde{\mathbf{P}}_{j}] = \mathcal{L}_j([\mathbf{W}_{j-1}, \widetilde{\mathbf{P}}_{j-1}]) \quad j = D+1,\ldots,K.
\end{equation}


\subsubsection{Instance-Conditioned Prompting}

Prompts play a crucial role in regulating the functionality of models~\cite{SAA,coCoOp}, serving as a mechanism to guide their performance. In this context, AdaCLIP introduces an instance-conditioned prompting method aimed at generating prompts based on input samples. This approach dynamically adjusts models to better suit the characteristics of the inputs, thereby enhancing the model's adaptability to new, unseen data, or anomalous patterns. Formally, it can be expressed as follows,

\begin{equation}
\label{eq:generator}
\mathbf{P}_{i}^{IC}, \widetilde{\mathbf{P}}_{i}^{IC} = \text{G}(\mathbf{I})
\end{equation}
where $\text{G}(\cdot)$ denotes a lightweight instance-conditioned prompts generator, and $\mathbf{P}_{i}^{IC} \in \mathrm{R}^{L \times d_v}, \widetilde{\mathbf{P}}_{i}^{IC} \in \mathrm{R}^{L \times d_l}$ are generated instance-conditioned vision and text prompts.

The introduction of dynamic prompts provides the model with heightened flexibility. This adaptability proves essential when confronting novel situations or encountering anomalous patterns. Moreover, the synergy of these dynamic prompts empowers the model to not only learn invariances of abnormalities but also adapt to the specific variances of each individual sample.

The significance of instance-conditioned prompts becomes apparent in their role as facilitators of "customized" adjustments for individual inputs. This tailored approach proves particularly beneficial in handling individual differences and special cases, a critical aspect when dealing with diverse datasets and domains. In essence, the incorporation of instance-conditioned prompts equips the model with the means to navigate the intricacies of diverse data, enhancing its overall efficacy in anomaly detection.

\subsubsection{Task-Conditioned Prompting}
While instance-conditioned prompting contributes to a dynamic representation space, it is not without its challenges, particularly regarding the susceptibility to disturbances inherent in the prompting generation process. Specifically, these prompts rely on complex generation processes through the generator $\text{G}(\cdot)$, which can introduce noise, particularly when the input data itself is noisy or irregular. This noise may result in considerable fluctuations in model predictions between individual samples, undermining consistency. 
In response to these challenges, this study introduces a task-conditioned prompting technique aimed at establishing a foundational optimizing direction. The primary objective is to mitigate the influence of inherent noise in instance-conditioned prompting, thereby enhancing the reliability and robustness of the model's responses. 

In contrast to instance-conditioned prompts generated dynamically, these task-conditioned prompts $\mathbf{P}_{i}^{TC} \in \mathrm{R}^{L \times d_v}, \widetilde{\mathbf{P}}_{i}^{TC} \in \mathrm{R}^{L \times d_l}$ are optimized in the training process and fixed during testing. Task-conditioned prompts serve as the cornerstone for baseline representation space building within the model. These prompts capture universal invariances of abnormalities, facilitating a robust mechanism for generalization to new data and unseen scenarios. The universality they provide is crucial for handling novel categories and ensuring the model's ability to generalize. Hence, AdaCLIP combines instance- and task-conditioned prompts for more reliable and robust ZSAD,

\begin{equation}
\mathbf{P}_{i} = \mathbf{P}_{i}^{IC} + \mathbf{P}_{i}^{TC}, \widetilde{\mathbf{P}}_{i} = \widetilde{\mathbf{P}}_{i}^{IC} + \widetilde{\mathbf{P}}_{i}^{TC}
\end{equation}
where $\mathbf{P}_{i},  \widetilde{\mathbf{P}}_{i}$ are the final utilized prompts for the vision and text encoders, respectively.

% Instance-conditioned prompts empower the model to provide customized representation space for individual inputs, capturing the variances in abnormalities. This capability allows the model to discern unique features in individual samples, particularly those exhibiting uncommon or entirely unseen abnormal patterns in the training data. On the other hand, task-conditioned prompts are responsible for learning invariances of abnormalities that persist throughout the entire training dataset. This global perspective is crucial for establishing a solid foundation and promoting generalization in the model. The combined use of instance- and task-conditioned parameters presents a stable and flexible framework for ZSAD. AdaCLIP harnesses the advantages of both parameter types, enabling the model to effectively handle diverse data types while maintaining high accuracy and robustness.



\subsection{Hybrid Semantic Fusion}

Concerning the computation of anomaly scores $S$, prevailing anomaly detection methods typically either utilize the maximum value within anomaly maps $\mathbf{M}$~\cite{CDO,2023CaiDis} or derive scores based on the global image embedding~\cite{VAND, WinClip}. However, the maximum-value-based approach has shown vulnerability in scenarios with false alarms~\cite{CDO}, while the global embeddings often lack robust fine-grained semantics, leading to potential inaccuracies in anomaly scores~\cite{VAND}. Therefore, AdaCLIP proposes a Hybrid Semantic Fusion (HSF) module to calculate anomaly scores based on both fine-grained local and global semantics, amalgamating the strengths of both strategies. Specifically, as Fig.~\ref{fig:HSF} shows, HSF extracts local semantics through the embeddings that are most likely to be abnormal. Then, HSF fuses these fine-grained semantics with image representations that contain global semantics.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/figure4.png}
    \caption{details of HSF.}
    \label{fig:HSF}
\end{figure}

\subsubsection{Local Semantic Extraction}

Vision embeddings with relatively high anomaly scores are more likely to indicate abnormalities~\cite{CDO, wang2021student}. In simpler terms, these embeddings encapsulate intricate semantics associated with anomalies. To distill these semantics, HSF selects the top-K embeddings based on the corresponding anomaly map in individual layers. These selected embeddings typically represent various candidates for anomaly regions. However, directly fusing these embeddings may diminish the significance of regions with smaller scales. In order to apply similar attention to different regions, HSF proposes to extract their cluster centroids as the final embeddings for local semantics,

\begin{equation}
\label{eq:fusion}
\mathcal{S}_i = \text{Kmeans}(\text{TopK}(\mathbf{E}_i  | \mathbf{M}_{(x,y,1)}))
\end{equation}

Here, $\text{TopK}(\mathbf{E}_i  | \mathbf{M}_{(x,y,1)})$ denotes the selection of the top-K embeddings with the highest abnormal scores conditioned on anomaly maps $\mathbf{M}_{(x,y,1)}$. $\text{Kmeans}(\cdot)$ represents the Kmeans clustering algorithm, and $\mathcal{S}_i$ is the generated index set for individual clusters.

Subsequently, the $j$-th cluster centroid in the $i$-th layer is calculated by averaging its corresponding embeddings,

\begin{equation}
\mathbf{C}_{i,j} = \frac{1}{|\mathcal{S}_{i,j}|} \sum_{k \in \mathcal{S}_{i,j}}{\mathbf{E}_{i,k}}
\end{equation}

The local semantic ${\mathbf{C}}_i$ for the $i$-th layer is obtained by averaging the cluster centroids,

\begin{equation}
{\mathbf{C}}_{i} = \frac{1}{N_c} \sum_{j = 0}^{N_c}{\mathbf{C}_{i,j}}
\end{equation}


\subsubsection{Local-Global Semantic Aggregation}
Image representations $\mathbf{F}^I$ encapsulate global semantics for the inputs, proving beneficial for anomaly score calculation~\cite{WinClip}. In this context, HSF integrates global image representations with the previously discussed local semantics to create enriched image representations. Specifically, the local semantics are projected to the common V-L representation space through the aforementioned projection layer $\text{P}(\cdot)$ before the aggregation, 

\begin{equation}
\widetilde{\mathbf{F}}^I = \mathbf{F}^I + \sum_{i \in \mathcal{H}} {\text{P}({\mathbf{C}}_{i})}
\end{equation}

Here, $\widetilde{\mathbf{F}}^I$ signifies the resulting hybrid semantic representation, subsequently employed for calculating anomaly scores using Equation~\ref{eq:AS}.

\subsection{Training and Inference}

During the training stage, the parameters of the CLIP model are frozen. AdaCLIP only optimizes the hybrid multi-modality prompts and the project layers. Focal loss~\cite{focalloss} is utilized for anomaly score calculation.  Focal loss and dice loss~\cite{diceloss} are employed to produce reliable anomaly maps. During inference, the anomaly score and maps are derived from Equations~\ref{eq:AS} and ~\ref{eq:AM}, respectively.


